SN 2022ann: A type Icn supernova from a dwarf galaxy that reveals helium in its circumstellar environment

We present optical and near-infrared (NIR) observations of the Type Icn supernova (SN Icn) 2022ann, the fifth member of its newly identified class of SNe. Its early optical spectra are dominated by narrow carbon and oxygen P-Cygni features with absorption velocities of 800 km/s; slower than other SNe Icn and indicative of interaction with a dense, H/He-poor circumstellar medium (CSM) that is outflowing slower than a typical Wolf-Rayet wind velocity of $>$1000 km/s. We identify helium in NIR spectra obtained two weeks after maximum and in optical spectra at three weeks, demonstrating that the CSM is not fully devoid of helium. We never detect broad spectral features from SN ejecta, including in spectra extending to the nebular phase, a unique characteristic among SNe~Icn. Compared to other SNe Icn, SN 2022ann has a low luminosity, with a peak o-band absolute magnitude of -17.7, and evolves slowly. We model the bolometric light curve and find it is well-described by 1.7 M_Sun of SN ejecta interacting with 0.2 M_sun of CSM. We place an upper limit of 0.04 M_Sun of Ni56 synthesized in the explosion. The host galaxy is a dwarf galaxy with a stellar mass of 10^7.34 M_Sun (implied metallicity of log(Z/Z_Sun) $\approx$ 0.10) and integrated star-formation rate of log(SFR) = -2.20 M_sun/yr; both lower than 97\% of the galaxies observed to produce core-collapse supernovae, although consistent with star-forming galaxies on the galaxy Main Sequence. The low CSM velocity, nickel and ejecta masses, and likely low-metallicity environment disfavour a single Wolf-Rayet progenitor star. Instead, a binary companion star is likely required to adequately strip the progenitor before explosion and produce a low-velocity outflow. The low CSM velocity may be indicative of the outer Lagrangian points in the stellar binary progenitor, rather than from the escape velocity of a single Wolf-Rayet-like massive star.

==> authors.tex <==
\author[K.~W.~Davis et al.]{
K.~W.~Davis,$^{1}$\thanks{E-mail: kywdavis@ucsc.edu}
K.~Taggart,$^{1}$
S.~Tinyanont,$^{1}$
R.~J.~Foley,$^{1}$
V.~A.~Villar,$^{2}$
C.~R.~Angus,$^{3}$
D.~A.~Coulter,$^{1}$
N.~Earl,$^{4}$
D.~Farias,$^{3}$
W.~V.~Jacobson-Galan,$^{5}$
D.~O.~Jones,$^{1,11,19}$
C.~D.~Kilpatrick,$^{6}$
D.~Langeroodi,$^{3}$
C.~Larison,$^{7}$
P.~McGill,$^{1}$
H.-Y.,~Miao,$^{8}$
C.~M.~Pellegrino,$^{13,14}$
C.~L.~Ransome,$^{2}$
S.~Rest,$^{9}$
A. Santos,$^{10}$
M.~R.~Siebert,$^{12}$
G.~Terreran.$^{13}$
S.~K.~Yadavalli,$^{2}$
K.~Auchettl
T.J.L.~de~Boer,$^{15}$
C.~R.~Bom,$^{10}$
K.~C.~Chambers,$^{15}$
A.~V.~Filippenko,$^{5}$
L.~Galbany,$^{16}$
H.~Gao,$^{15}$
D. A. Howell,$^{13,14}$
A.~Kanaan,$^{10}$
C.-C.~Lin,$^{15}$
E.~A.~Magnier,$^{15}$
Y.-C.~Pan,$^{8}$
T.~Ribeiro
A.~Rest,$^{9,12}$
W.~ Schoenell,$^{17}$
R.~J. Wainscoat,$^{15}$
Y.~Zenati,$^{15,18}$


\\
% List of institutions
$^{1}$Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 95064\\
$^{2}$Department of Astronomy \& Astrophysics, The Pennsylvania State University, University Park, PA 16802, USA} \affiliation{Institute for Computational \& Data Sciences, The Pennsylvania State University, University Park, PA, USA}\\
$^{3}$DARK, Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200 Copenhagen, Denmark\\
$^{4}$Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green St., IL 61801, USA\\
$^{5}$Department of Astronomy and Astrophysics, University of California, Berkeley, CA 94720, USA\\
$^{6}$Center for Interdisciplinary Exploration and Research in Astrophysics (CIERA) and Department of Physics and Astronomy, Northwestern University, Evanston, IL 60208, USA\\
$^{7}$Department of Physics and Astronomy, Rutgers, the State University of New Jersey,\\136 Frelinghuysen Road, Piscataway, NJ 08854-8019, USA\\
$^{8}$Graduate Institute of Astronomy, National Central University, 300 Zhongda Road, Zhongli, Taoyuan 32001, Taiwan\\
$^{9}$Department of Physics and Astronomy, The Johns Hopkins University, Baltimore, MD 21218, USA\\
$^{10}$Centro Brasileiro de Pesquisas F\'isicas, Rua Dr. Xavier Sigaud 150, CEP 22290-180, Rio de Janeiro, RJ, Brazil\\
$^{11}$Gemini Observatory/NSF's NOIRLab, 670 N. A'ohoku Place, Hilo, Hawai'i, 96720, USA\\
$^{12}$Space Telescope Science Institute, Baltimore, MD 21218, USA\\
$^{13}$Las Cumbres Observatory, 6740 Cortona Drive, Suite 102, Goleta, CA 93117-5575, USA\\
$^{14}$Department of Physics, University of California, Santa Barbara, CA 93106-9530, USA\\
$^{15}$Institute for Astronomy, University of Hawaii, 2680 Woodlawn Drive, Honolulu, HI 96822, USA\\
$^{16}$Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Can Magrans, s/n, E-08193 Barcelona, Spain. $^{2}$Institut d’Estudis Espacials de Catalunya (IEEC), E-08034 Barcelona, Spain.\\
$^{17}$NOAO, P.O. Box 26732, Tucson, AZ 85726\\
$^{18}$ISEF Postdoctoral Fellow
$^{19}$einstein Fellow
